Gyrokinetic Continuum Simulation of Turbulence in Open-Field-Line Plasmas

The properties of the boundary plasma in a tokamak are now recognized to play a key role in determining the achievable fusion power and the lifetimes of plasma-facing components. Accurate quantitative modeling and improved qualitative understanding of the boundary plasma ultimately require five-dimensional gyrokinetic turbulence simulations, which have been successful in predicting turbulence and transport in the core. The additional challenges of boundary-plasma simulation necessitate the development of new gyrokinetic codes or major modifications to existing core gyrokinetic codes. In this thesis, we develop the first gyrokinetic continuum code capable of simulating plasma turbulence on open magnetic field lines, which is a key feature of a tokamak scrape-off layer. In contrast to prior attempts at this problem, we use an energy-conserving discontinuous Galerkin discretization in space. To model the interaction between the plasma and the wall, we design conducting-sheath boundary conditions that permit local currents into and out of the wall. We start by designing spatially one-dimensional kinetic models of parallel SOL dynamics and solve these systems using novel continuum algorithms. By generalizing these algorithms to higher dimensions and adding a model for collisions, we present results from the first gyrokinetic continuum simulations of turbulence on two types of open-field-line systems. The first simulation features uniform and straight field lines, such as found in some linear plasma devices. The second simulation is of a hypothetical model we developed of the NSTX scrape-off layer featuring helical field lines. These developments comprise a major step towards a gyrokinetic continuum code for quantitative predictions of turbulence and transport in the boundary plasma of magnetic fusion devices.

==> ch-appendicies/code.tex <==
\chapter{Supplementary Code\label{ch:supplementary-code}}

The code in this section makes extensive use of a
Lua function \texttt{runUpdater}, which we define as
\begin{lstlisting}[language={[5.2]Lua}]
function runUpdater(updater, currTime, timeStep, inpFlds, outFlds)
   updater:setCurrTime(currTime)
   if inpFlds then
      updater:setIn(inpFlds)
   end
   if outFlds then
      updater:setOut(outFlds)
   end
   return updater:advance(currTime+timeStep)
end
\end{lstlisting}

\section{Limiter Bias Modifications}
To model limiter biaising in the 3D2V LAPD simulations of Section \ref{ch:lapd},
a 3D potential field is created in the Lua script and set to have the value 0 along field lines
that do not intersect the biasable limiter and $V_{\mathrm{bias}}$ along field lines that do.
The following code block creates the bias field $\phi_\mathrm{bias}$, which is the variable \texttt{phiOffset}.

\begin{lstlisting}[language={[5.2]Lua}]
initPhiOffset = Updater.EvalOnNodes3D {
  onGrid = grid_3d,
  basis = basis_3d,
  shareCommonNodes = false,
  evaluate = function(x,y,z,t)
    local r = math.sqrt(x^2 + y^2)
    if r >= r_s then
      return V_bias
    else
      return 0
    end
  end
}
-- offset potential for sheath bc
phiOffset = DataStruct.Field3D {
   onGrid = grid_3d,
   numComponents = basis_3d:numNodes(),
   ghost = {1, 1},
}
runUpdater(initPhiOffset, 0, 0, {}, {phiOffset})
\end{lstlisting}

The \texttt{phiOffset} field is then combined with the electrostatic potential that is
the solution of the gyrokinetic Poisson equation (labeled as \texttt{phi3d}) into the
sheath potential field \texttt{phiSheath}, which is used in the sheath-model boundary conditions.
The following code shows how this procedure is implemented in the function that applies
boundary conditions to the distribution functions.

\begin{lstlisting}[language={[5.2]Lua}]
function applyBcToDistF(tCurr, myDt, fElc, fIon, phiIn)
  fIon:sync()
  fElc:sync()
  -- apply zero inflow boundary conditions in z to ions
  runUpdater(bcLowerZIon, tCurr, myDt, {}, {fIon})
  runUpdater(bcUpperZIon, tCurr, myDt, {}, {fIon})
  -- apply zero inflow boundary conditions in z to electrons
  runUpdater(bcLowerZElc, tCurr, myDt, {}, {fElc})
  runUpdater(bcUpperZElc, tCurr, myDt, {}, {fElc})
  -- compute potential for sheath bc
  phiSheath:combine(1.0, phiIn, -1.0, phiOffset)
  -- apply biased sheath boundary conditions to electron distribution
  -- function
  runUpdater(biasedSheathElcCalc, tCurr, myDt, {phiSheath,
    hamilDerivKeElc}, {fElc})
  -- apply biased sheath boundary conditions to ion distribution 
  -- function
  runUpdater(biasedSheathIonCalc, tCurr, myDt, {phiSheath,
    hamilDerivKeIon}, {fIon})
  -- sync cells in distribution function 
  fElc:sync()
  fIon:sync()
end
\end{lstlisting}


==> ch-appendicies/post-processing.tex <==
\chapter{Post-Processing Methods}
In this section, we document the post-processing methods employed elsewhere in this thesis.
\hl{Plotting, Fourier transforms, correlation functions}

